Molecular Shattering

Recent observations suggest galaxies may ubiquitously host a molecular component to their multiphase circumgalactic medium (CGM). However, the structure and kinematics of the molecular CGM remains understudied theoretically and largely unconstrained observationally. Recent work suggests molecular gas clouds with efficient cooling survive acceleration in hot winds similar to atomic clouds. Yet the pressure-driven fragmentation of molecular clouds when subjected to external shocks or undergoing cooling remains unstudied. We perform radiative, inviscid hydrodynamics simulations of clouds perturbed out of pressure equilibrium to explore the process of hydrodynamic fragmentation to molecular temperatures. We find molecular clouds larger than a critical size can shatter into a mist of tiny droplets, with the critical size deviating significantly from the atomic case. We find that cold clouds shatter only if the sound crossing time exceeds the local maximum of the cooling time ~8000 K. Moreover, we find evidence for a universal mechanism to 'shatter' cold clouds into a 'mist' of tiny droplets as a result of rotational fragmentation -- a process we dub 'splintering.' Our results have implications for resolving the molecular phase of the CGM in observations and cosmological simulations.

==> tables/coolingTable.tex <==
\begin{table}
\caption{\label{tab:cooling}Piece-wise Power Law Fit to the Cooling Curve.}
\begin{tabular}{ c c r }
\hline
 Temperature Range & Coefficient (erg cm$^3$ s$^{-1}$) & Index \\ 
 \hline
 300\,K $\leq$ T $<$ 2000\,K & $10^{-26}$ & 0.2 \\  
 2000\,K $\leq$ T $<$ 8000\,K & $1.5 \times 10^{-26}$ & 0.5 \\
 8000\,K $\leq$ T $<$ $10^4$\,K & $3 \times 10^{-26}$ & 19.6 \\
 $10^{4}$\,K $\leq$ T $< 2 \times 10^{4}$\,K & $2.4 \times 10^{-24}$ & 6 \\
 $2 \times 10^{4}$\,K $\leq$ T $< 2 \times 10^{5}$\,K & $1.5438 \times 10^{-24}$ & 0.6 \\
 $2 \times 10^{5}$\,K $\leq$ T $< 1.5 \times 10^{6}$\,K & $6.6831 \times 10^{-22}$ & -1.7 \\ 
 $1.5 \times 10^{6}$\,K $\leq$ T $< 8 \times 10^{6}$\,K & $2.7735 \times 10^{-23}$ & -0.5 \\
 $8 \times 10^{6}$\,K $\leq$ T  $< 5.8 \times 10^{7}$\,K & $1.1952 \times 10^{-23}$ & 0.22 \\
 $5.8 \times 10^{7}$\,K $\leq$ T & $1.8421 \times 10^{-23}$ & 0.4 \\ 
 
\hline
\end{tabular}
\end{table}

==> tables/table_cloudSizes.tex <==
\begin{table}
\caption{\label{tab:definitions}Notation.}
\begin{tabular}{ l r }
\hline
 Name & Property \\ 
 \hline
 \lrg & 100\,pc \\  
 \med & 10\,pc \\
 \sml & 0.01\,pc \\
 cold & $\sim$10$^{3}$ K \\
 warm & $\sim$10$^{4}$ K \\
 hot  & $\sim$10$^{6}$ K \\
 \Tmix & \big(\Tcl$\,$\Twind\big)$^{1/2}$ \\
 \tmixCool & $t_{\rm cool}$ \big(T = \Tmix\big) \\
 \tmax & max\big($t_{\rm cool}$ (T < \Tmix)\big) \\
 \tminmix & $t_{\rm cool}$ \big($\sqrt{T(\rm min(t_{\rm cool})) \Twind}$\big) \\ 
 
\hline
\end{tabular}
\end{table}

==> tables/table_flashParams.tex <==
\begin{table}
\caption{Simulation parameters.}
\label{tab:flashParams}
\begin{tabular}{ l c }
\hline
 Parameter Name & Parameter Value \\ 
 \hline
 RiemannSolver & HLLC \\  
 slopeLimiter & mc \\
 order & 2$^a$ \\
 charLimiting & False$^b$ \\
 use\_hybridOrder & True \\
 hybridorderkappa & 0.5 \\
 cfl & 0.2 \\
\hline
\end{tabular}

$a$. MUSCL-Hancock,\\
$b$. Reconstruction in the primitive variables.
\end{table}

==> tables/table_runList.tex <==
\providecommand{\fourEfour}{$4 \times 10^{4}$}
%\newcommand{\fourEThree}{$4 \times 10^{3}$}
%\newcommand{\eightEThree}{$8 \times 10^{3}$}
%\newcommand{\tenFive}{$10^{5}$}
%\newcommand{\tenFour}{$10^{4}$}
%\newcommand{\tenThree}{$10^{3}$}

\begin{table*}
\caption{\label{tab:ListOfRuns}Run parameters.}
\begin{tabular}{rrrrrrr}
\toprule
$\chi_{\rm F}$ & T$_{\rm fl}$\,(K) &  $r_{\rm cl}$ (pc) &  $r_{\rm cl} / l_{\rm sh}$ &  atomically shattered & molecularly shattered \\
\midrule
                     10$^2$ & 4 $\times 10^5$ &                 0.04 &                 3.87 &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                 0.32 &                 30.0 &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                  2.5 &                  232 &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                 19.3 &                 1800 &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                  150 &    $1.4 \times 10^4$ &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                 1160 &               $10^5$ &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &                 9000 &      $8 \times 10^5$ &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   No & N/A \\
                     10$^2$ & 4 $\times 10^5$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   No & N/A \\
                     215 & 1.86 $\times 10^5$ &                 0.32 &                 30.0 &   No & N/A \\
                     215 & 1.86 $\times 10^5$ &                  2.5 &                  232 &   Yes & N/A \\
                     215 & 1.86 $\times 10^5$ &                 19.3 &                 1800 &   Yes & N/A \\
                     215 & 1.86 $\times 10^5$ &                  150 &    $1.4 \times 10^4$ &   Yes & N/A \\
                     215 & 1.86 $\times 10^5$ &                 1160 &               $10^5$ &   Yes & N/A \\
                     215 & 1.86 $\times 10^5$ &                 9000 &      $8 \times 10^5$ &   No & N/A \\
                     215 & 1.86 $\times 10^5$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   No & N/A \\
                     464 & 8.62 $\times 10^4$ &                 0.32 &                 30.0 &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &                  2.5 &                  232 &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &                 19.3 &                 1800 &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &                  150 &    $1.4 \times 10^4$ &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &                 1160 &               $10^5$ &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &                 9000 &      $8 \times 10^5$ &   Yes & N/A \\
                     464 & 8.62 $\times 10^4$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   No & N/A \\
                     464 & 8.62 $\times 10^4$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   No & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                 0.04 &                 3.87 &   No & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                 0.32 &                 30.0 &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                  2.5 &                  232 &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                 19.3 &                 1800 &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                  150 &    $1.4 \times 10^4$ &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                 1160 &               $10^5$ &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &                 9000 &      $8 \times 10^5$ &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   Yes & N/A \\
                     10$^3$ & 4 $\times 10^4$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   No & N/A \\
                      2150 & 1.86 $\times 10^4$ &                 0.32 &                 30.0 &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &                  2.5 &                  232 &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &                 19.3 &                 1800 &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &                  150 &    $1.4 \times 10^4$ &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &                 1160 &               $10^5$ &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &                 9000 &      $8 \times 10^5$ &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   Yes & N/A \\
                      2150 & 1.86 $\times 10^4$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                 0.04 &                 3.87 &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                 0.32 &                 30.0 &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                  2.5 &                  232 &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                 19.3 &                 1800 &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                  150 &    $1.4 \times 10^4$ &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                 1160 &               $10^5$ &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &                 9000 &      $8 \times 10^5$ &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &      $7 \times 10^4$ &      $6 \times 10^6$ &   Yes & N/A \\
                      4640 & 8.62 $\times 10^3$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   Yes & N/A \\
                      10$^4$ & 4 $\times 10^3$ &                 0.32 &                 30.0 &   No & No \\
                      10$^4$ & 4 $\times 10^3$ &                  2.5 &                  232 &   Yes & No \\
                      10$^4$ & 4 $\times 10^3$ &                 19.3 &                 1800 &   Yes & Yes \\
                      10$^4$ & 4 $\times 10^3$ &                  150 &    $1.4 \times 10^4$ &   Yes & Yes \\
                      10$^4$ & 4 $\times 10^3$ &                 1160 &               $10^5$ &   Yes & Yes \\
                      10$^4$ & 4 $\times 10^3$ &                 9000 &      $8 \times 10^5$ &   Yes & Yes \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                 0.32 &                 30.0 &   Yes & No \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                  2.5 &                  232 &   Yes & No \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                 19.3 &                 1800 &   Yes & No \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                  150 &    $1.4 \times 10^4$ &   Yes & Yes \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                 1160 &               $10^5$ &   Yes & Yes \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &                 9000 &      $8 \times 10^5$ &   Yes & Yes \\
                      2.15 $\times 10^4$ & 1.86 $\times 10^3$ &      $5 \times 10^5$ &      $5 \timex 10^7$ &   Yes & Yes \\
                      4.64 $\times 10^4$ & 862 &                 0.32 &                 30.0 &   Yes & No \\
                      4.64 $\times 10^4$ & 862 &                  2.5 &                  232 &   Yes & No \\
                      4.64 $\times 10^4$ & 862 &                 19.3 &                 1800 &   Yes & No \\
                      4.64 $\times 10^4$ & 862 &                  150 &    $1.4 \times 10^4$ &   Yes & Yes \\
                      4.64 $\times 10^4$ & 862 &                 1160 &               $10^5$ &   Yes & Yes \\
                      4.64 $\times 10^4$ & 862 &      $7 \times 10^4$ &      $6 \times 10^6$ &   Yes & Yes \\
                      10$^5$ & 400 &                  2.5 &                  232 &   No  & No \\
                      10$^5$ & 400 &                 19.3 &                 1800 &   Yes & Yes \\
                      10$^5$ & 400 &                  150 &    $1.4 \times 10^4$ &   Yes & Yes \\
                      10$^5$ & 400 &                 1160 &               $10^5$ &   Yes & Yes \\
                      10$^5$ & 400 &                 9000 &      $8 \times 10^5$ &   Yes & Yes \\
                      10$^5$ & 400 &      $7 \times 10^4$ &      $6 \times 10^6$ &   Yes & Yes \\
\bottomrule
\end{tabular}

Note that we used $n_{\rm cl}$ = 0.1 \cc\, $T_{\rm cl}$ = $4 \times 10^5$, $chi_{\rm i} = 100$, and $T_{\rm hot} = 4 \times 10^7$ for an initial pressure of $P = 4 \times 10^4$ in all simulations, whereas one may scale up the density (and linearly scale down the radius) by $\sim$100 for conditions representative of the central regions of galaxy clusters.
\end{table*}
